Octocopter Design: Modelling, Control and Motion Planning

This book provides a solution to the control and motion planning design for an octocopter system. It includes a particular choice of control and motion planning algorithms which is based on the authors' previous research work, so it can be used as a reference design guidance for students, researchers as well as autonomous vehicles hobbyists. The control is constructed based on a fault tolerant approach aiming to increase the chances of the system to detect and isolate a potential failure in order to produce feasible control signals to the remaining active motors. The used motion planning algorithm is risk-aware by means that it takes into account the constraints related to the fault-dependant and mission-related maneuverability analysis of the octocopter system during the planning stage. Such a planner generates only those reference trajectories along which the octocopter system would be safe and capable of good tracking in case of a single motor fault and of majority of double motor fault scenarios. The control and motion planning algorithms presented in the book aim to increase the overall reliability of the system for completing the mission.

==> chapters/Chapter5/ch5.tex <==
\chapter{Fault-tolerant control\label{chap:Metode-upravljanja-otporno-na-kvarove}}


Kako je već rečeno u 4. poglavlju
 \color{red}
regardless of whether the configuration of a MAV is redundant, the control algorithm has a significant role in improving fault-tolerance of the MAV system. If a control algorithm is fault-ignorant, having redundant components does not necessarily increase the reliability of the MAV system or the probability of completing the mission. The control algorithms that inherently possess a certain level of robustness with respect to possible failures increase the reliability of the system.

 \color{black}


Zbog toga je u ovom poglavlju ukratko prezentirano područje upravljanja
otpornog na kvarna stanja (\emph{engl.} Faul-tolerant control), od
kratkog pregleda povijesnog razvoja do objašnjenja osnovne terminologije
koja se koristi u području upravljanja otpornog na kvarna stanja.
Takodjer, opisana je procedura projektiranja jednostavnog PD regulatora
koji kombiniranjem s metodom koja za identifikaciju i izolaciju nastalog
kvarnog stanja (zasnovana na metodi najmanjih kvadrata) tvori regulator
otporan na nastanak kvarnog stanja. Procedura je publicirana u radu
\cite{Osmic_AIM}.


\medskip{}


\section{Povijesni razvoj upravljanja otpornog na kvarna stanja}

Razvoj upravljanja otpornog na kvarna stanja potaknut je nizom industrijskih
i zrakoplovnih nesreća koje su se dogodile tijekom prošloga stoljeća.
Neke od nesreća koje su imale pogubne posljedice po ljudske živote
i okoliš su: curenje radioaktivnog materijala na drugom reaktoru nuklearne
elektrane ``Three miles island''\cite{Tri_milje_island}, nuklearne
nesreće u Černobilu \cite{Cernobil_2} i Fokušimi \cite{fukushima}
te veći broj zrakoplovnih nesreća \cite{FTC_Review_patton2015fault}
koje su za posljedicu imale gubitak ljudskih života, a čiji uzroci
nisu bili ljudski faktor nego otkazivanje pojedinih dijelova sustava.
U radovima \cite{Statistika_nesreca} i \cite{Nesrece_Report} navodi
se da je većina zrakoplovnih nesreća povezana s gubljenjem upravljivosti
letjelica tijekom leta. Zbog navedenih razloga jako je bitno da je
upravljački sustav u stanju prepoznati da je došlo do nastanka kvarnog
stanja, te da se potom pokuša s nastalim kvarnim stanjem izboriti
u optimalnom smislu, tako da se sustavom nastavi upravljati na siguran
način, naravno uz smanjenje njegovih performansi.

Interes za područje upravljanja otpornog na kvarna stanja porastao
je ranih sedamdesetih godina prošlog stoljeća u kemijskoj industriji.
Razvijene su različite metode koje su dobile zajednički termin ``otkrivanje
i lokalizacija kvarnog stanja zasnovane na matematičkom modelu''.
Teorija u području upravljanja otpornog na kvarna stanja, kao i zaključci
koji su izvedeni iz teorije upravljanja otpornog na kvarna stanja,
preuzeti su i doradjeni od zrakoplovne-industrije. 


\color{red}
In the aviation industry, the term "physical redundancy" was introduced, which represent the real-time measurement of a variable of interest (altitude, pressure, flight speed, aircraft inclination, rudder rotation state) with multiple sensors (usually three or four) with different technologies, to prevent the possibility of the occurrence of the same fault on the same type of sensor. All measured values are compared and, for significantly deviates between obtained values, that sensor is no longer taken into account. However, the probability of simultaneous failure of two or more sensors is less than the probability of failure of only one, so this type of decision-making is called "majority voting". Also, if all sensors give a value that is outside the normal range then, it is more likely, that it is a structural failure than that all sensors have failed at the same time. In addition to physical redundancy, there is the so-called analytical redundancy that does not require the installation of additional components but it calculates each parameter that is relevant to the functioning of the system analytically based on available measurements of the system. When the system is in normal mode (fault-free state), the parameters are measured and compared does it give similar values as analytically calculated system states. In the case when a failure occurs on one of the subsystems, the values obtained by measurement (using sensors) and those obtained analytically are different. Choosing appropriate analytical method and the state of the system to be measured, it is possible to distinguish the locations of the fault as well as to identify the fault, i.e. to determine whether the fault occurred on the sensor, actuator or structural failure. Physical redundancy can increase the reliability of the aircraft, but on the other hand, it requires higher costs and more complexity in the implementation of the desired system. Methods (physical or analytical) that can be performed to identify the occurrence of a fault in the system are part of the methods of fault detection.

\color{black}




U području upravljanja otpornog na kvarna stanja za klasu linearnih
sustava razvijeni su različiti pristupi i strategije za identifikaciju
i lokalizaciju kvarnog stanja, kao što su pristupi zasnovani na obzerverima,
parametarskoj estimaciji, jednadžbama pariteta, upotrebi Kalmanova
filtra i sl. Ključne reference za klasu upravljanja otpornog na kvarna
stanja kod linearnih sustava mogu se naći u radovima \cite{FTC_Review_patton2015fault},
\cite{Kniga_paton_chen2012robust}, \cite{isermann1997trends}, \cite{isermann2006fault_knjiga},
\cite{pouliezos2013real}. Takodjer, za klasu nelinearnih sustava razvijene
su metode zasnovane na matematičkom modelu \cite{Kniga_paton_chen2012robust},
\cite{astrom2011control}, \cite{seliger1991fault}, \cite{zhirabok1997fault}.
Za razliku od metoda koje se zasnivaju na točnom poznavanju matematičkog
modela razvijene su i metode koje ne zahtijevaju matematički model.
U te metode spadaju metode zasnovane na neuronskim mrežama \cite{Kniga_paton_chen2012robust}
i neizrazitoj logici \cite{AI_frank1996analytical}. Prednost tih
metoda zasniva se na činjenici da nije nužno poznavati analitički
model sustava kojim se želi upravljati. Dovoljno je poznavati samo
veze izmedju pojedinih dijelova sustava bez potrebe za znanjem analitičkog
oblika podsustava. Kod takvog pristupa uzroci i posljedice nastanka
kvarnog stanja mogu se lakše opisati.

Zadatak je upravljanja otpornog na kvarna stanja zadržati nazivno
ponašanje sustava bez obzira na varijacije u parametrima sustava,
a koje mogu biti posljedica kvarnoga stanja. Dobar pregled literature
i osnovni koncepti upravljanja otpornog na kvarna stanja dani su u
preglednom radu \cite{zhang2008bibliographical}. U radu je predložena
i klasifikacija metoda za rekonfiguraciju upravljanja otpornog na
kvarna stanja prikazane su matematičke metode te su navedeni alati
koji se mogu koristiti. 

\section{Terminologija u području upravljanja otpornog na kvarna stanja}

Budući da se područje upravljanja otpornog na kvarna stanja počelo
intenzivnije razvijati tijekom sedamdesetih i osamdesetih godina prošloga
stoljeća postojale su različite definicije kvarnih stanja i načina
reagiranja na pojavu kvarnog stanja. S ciljem ujednačenja terminologije,
IFAC-ov tehnički komitet SAFEPROCESS (\emph{engl.} \emph{IFAC Technical
Committee: SAFEPROCESS Fault Detection, Supervision and Safety for
Technical Processes}) pokrenuo je inicijativu za definiranje osnovnih
termina u ovome području. Na tu je temu organiziran niz simpozija
(Baden-Baden(1991), Helsinki (1994), Hull (1994), Budapest (2000),
Washington(2003), Bejing (2006)) i radionica (Kyoto (1986), Newark
(1992), Newcastle (1995), Folaize (1998), Cheju (2001)). Revidirana
inačica terminologije koja je nastala kao rezultat tih simpozija i
radionica može se sažeti u sljedećem \cite{isermann2006fault_knjiga}:




\medskip{}
\color{red}
\begin{itemize}
\item \textbf{Fault} - "A fault is an unpermitted deviation of at least one characteristic property (feature) of the system from the acceptable, usual, standard condition."
\item \textbf{Failure}  - "A failure is a permanent interruption of a system's ability to perform a required function under specified operating conditions."
\item \textbf{Malfunction}  - "A malfunction is a intermittent irregularity in the fulfillment of a system's desired function." 
\item \textbf{Reliability}  - "Ability of a system to perform a required function under stated conditions, within a given scope, during a given period of time." 
\item \textbf{Safety}  - "Ability of a system not to cause danger to person or equipment or the environment."
\item \textbf{Availability}  - "Probability that a system or equipment will operate satisfactorily and effective at any period of time." 
\item \textbf{Dependability} - "A form of availability that has the property of always being available when required (and not at any time)."
\item \textbf{Integrity}  - "The integrity of a system is the ability to detect faults in its own operation and to inform a human operator."
\item \textbf{Safety integrity} - "Safety integrity is the probability of a safety-related system satisfactora performing the required safety function under all the stated conditions within a period of time." 
\item \textbf{Hazard}  - "Hazards are undesirable system conditions with the potential to cause or to contribute to damage or accident with injuries, death, material damage or environmental pollution .''
\item \textbf{Risk}  - "Represents a combination of the likelihood of the hazard and its severity to operators or the environment."
\item \textbf{Maintainability}  - "Maintainability is a quality of several features which enable a system to be maintained. This includes proper design, required tools, standardized components, group subsystems (modularity), aids for trouble-shoting, space and logistics. "
\item \textbf{Robustness}  - "The ability of the system to maintain satisfactory performance in the event of a change in system parameters." 
\item \textbf{Fault Detection } - ``Determination of faults present in a system and time of detection''.
\item \textbf{Residual } - ``Fault indicator, based on deviations between measurements and model-equation-based calculations.
When the system is not in a faulty-state the residual is approximately equal to zero, it deviates significantly from zero in the faulty-state condition.''
\color{red}
\item \textbf{Fault Isolation}  - ``Determination of kind, location and time of detection of a fault by evaluating symptoms. Follows fault detection''.
\item \textbf{Fault Identification} - ``Determination of the size and time-variant behavior of a
fault. Follows fault isolation.''
\item \textbf{Fault Diagnosis} - ``Determination of kind, size, location and time of detection
of a fault by evaluating symptoms. Follows fault detection.
Includes fault detection, isolation and identification.''
\item \textbf{Fault accomodation}  - ``Change controller parameters or controller structure. Decrease performance, e.g., reduce through-put of the controlled system. Change settings in the surrounding process to decrease the requirements to the controlled system.''
\color{red}
\item \textbf{Fault tolerance} - ``Property that enables a system to continue operating properly in the event of the failure of one or more faults within some of its components with a permitted reduction in nominal performance.''
\end{itemize}
\color{black}
\section{Pregled metoda dijagnostike kvarnih stanja i metoda upravljanja otpornih
na njih }

Standardna struktura sustava kojim je potrebno upravljati prikazana
na slici \ref{fig:rekonfiguracija}. Kvarno stanje u sustavu može
nastati na bilo kojoj komponenti sustava (aktuator, senzor, strukturalna
komponenta ili bilo koja kombinacija navedenih komponenata) i u bilo
koje vrijeme. S obzirom na navedeno, može se izvršiti klasifikacija
kvarnih stanja po različitim kriterijima. Tako možemo govoriti o vremenskoj
distribuciji i fizičkoj lokaciji kvarnih stanja ili o djelovanjima
koje je kvarno stanje proizvelo u sustavu. Ako se radi o fizičkoj
lokaciji nastanka kvarnog stanja \cite{Active_FTC_zhang2002} onda
se kvarna stanja mogu razvrstati na:\medskip{}

\begin{figure}
\begin{centering}
\includegraphics[scale=0.6]{chapters/Chapter5/figures/rekonfiguracijska shema.pdf}
\par\end{centering}
\caption{Mehanizam rekonfiguracije kod aktivnih metoda upravljanja otpornog
na kvarna stanja \cite{Kniga_paton_chen2012robust}. 
\label{fig:rekonfiguracija}}
\end{figure}
\begin{itemize}
\item \textbf{Kvarno stanje na aktuatoru}, može biti zaglavljivanje (aktuator
je zaglavljen u nekoj od pozicija i vrijednost mu se ne može promijeniti),
djelomični ili potpuni otkaz upravljanja (aktuator reagira na upravljačke
akcije ali sa smanjenom efektivnošću, dok kod potpunog otkaza aktuator
više nema nikakve funkcionalnosti). 
\item \textbf{Kvarno stanje na senzoru}, podrazumijeva pogrešne ili nepostojeće
mjerne vrijednosti, a koje su posljedica izgaranja na elektroničkim
sklopovima senzora ili na pretvaraču.
\item \textbf{Strukturalno kvarno stanje}, podrazumijeva kvarno stanje na
samoj strukturi sustava kojim se upravlja, što dovodi do promjene
u dinamici sustava pa upravljanje više nije optimalno podešeno ili
može postati neodgovarajuće.
\end{itemize}
\medskip{}

U ovoj se disertaciji razmatraju kvarna stanja koja nastaju na sustavu
aktuatora, odnosno u našem slučaju na pogonskim motorima.

\subsection{Podjela metoda upravljanja otpornog na kvarna stanja }

Kod projektiranja sustava otpornog na kvarna stanja postoje dva pristupa,
odnosno dvije grupe metoda\cite{podjela_metoda_alwi2011fault}: (i)
pasivne metode i (ii) aktivne metode, kako je prikazano na slici \ref{aktivne i pasivne metode}.
Osnovna je odlika\textbf{ pasivnih metoda} da se još tijekom projektiranja
regulatora uzima u obzir nesigurnost modela sustava, odnosno regulator
se projektira za cijelu klasu mogućih sustava. Osnovni je nedostatak
pasivnih metoda da nisu u stanju izvršiti efektivno upravljanje \cite{FTC_Review_patton2015fault},
\cite{Kniga_paton_chen2012robust}, \cite{zhang2008bibliographical}. 

Za razliku od pasivnih metoda, \textbf{aktivne metode} reagiraju na
širu klasu kvarnih stanja koje se mogu pojaviti u sustavu. Aktivne
metode posjeduju mehanizam za otkrivanje i identifikaciju tipa kvarnog
stanja, te se pomoću mehanizma za rekonfiguraciju adaptiraju na nastalo
kvarno stanje u smislu da se zadrži stabilnost sustava uz smanjenje
nazivne performanse sustava. Osnovna shema aktivnih metoda prikazana
je na slici \ref{fig:rekonfiguracija}. 

\begin{figure}
\begin{centering}
\includegraphics[scale=0.55]{chapters/Chapter5/figures/FTC_upravljanje.pdf}
\par\end{centering}
\caption{Podjela metoda upravljanja otpornog na kvarna stanja \cite{podjela_metoda_alwi2011fault}.}
\label{aktivne i pasivne metode}
\end{figure}

U disertaciji se koristi aktivni pristup dijagnostike kvarnih stanja.
Za dijagnosticiranje kvarnih stanja postoje različite metode. Neke
su zasnovane na matematičkom modelu (\emph{engl.} Model-Based methods),
neke na znanju o sustavu bez poznavanja matematičkih relacija koje
vrijede u sustavu (\emph{engl.} Knowledge based), a postoje i metode
zasnovane na podacima (signalima) koji su dostupni o sustavu (\emph{engl.}
Proces history based methods), slika \ref{Dijagnoza kvara}. Detaljan
opis navedenih metoda može se naći u \cite{zhang2008bibliographical,venkatasubramanian2003review_I,venkatasubramanian2003review_II,venkatasubramanian2003review_III}.

\begin{figure}
\centering{}\includegraphics[scale=0.4]{chapters/Chapter5/figures/Metode_za_ident_kvara.pdf}
\caption{Podjela metoda za dijagnostiku kvarnih stanja \cite{zhang2008bibliographical}.}
\label{Dijagnoza kvara}
\end{figure}

Za svaku od prikazanih metoda na slici \ref{Dijagnoza kvara}, neophodno
je neko znanje o sustavu. U ovoj se disertaciji koriste metode zasnovane
na matematičkom metodu pa se u sljedećem potpoglavlju ukratko opisuju
te metode.

\subsection{Dijagnostika kvarnog stanja na osnovi matematičkog modela}

Osnovni je problem kod metoda dijagnoze kvarnih stanja koje se ne
zasnivaju na matematičkom modelu zahtjev dodavanja dodatne opreme
u sustav što povećava njegovu cijenu i gabarite ili se zahtijevaju
dodatna skupa mjerenja. Ako se ne posjeduje dodatni novac za skupu
opremu ili gabariti sustava ne dopuštaju dodavanje dodatne opreme,
onda se mogu koristiti sva dostupna mjerenja u sustavu s kombiniranjem
znanja o tome kako sustav treba raditi. U literaturi se taj koncept
naziva analitičkom redundancijom (\emph{engl.} analitic redudancy).
Osnovna razlika izmedju fizičke i analitičke redundancije prikazana
je na slici \ref{analiticka i hardverska redudaca}\cite{Kniga_paton_chen2012robust}.

\begin{figure}
\begin{centering}
\includegraphics[scale=0.6]{chapters/Chapter5/figures/Redudancija.pdf}
\par\end{centering}
\caption{Prikaz koncepta analitičke i fizičke redundacije \cite{Kniga_paton_chen2012robust}.}
\label{analiticka i hardverska redudaca}
\end{figure}

Analitička redundancija zasniva se na korištenju relacija izmedju ulaza
i izlaza. Istovremeno se procesiraju signali koji su prisutni na ulazu
i izlazu u stvarni sustav kao i ulazi i izlazi koji se primjenjuju
na model. Potom se računa odstupanje (\emph{engl.} residual) izmedju
karakterističnih veličina stvarnoga sustava i njegova modela te se
dobiveni rezultat šalje u blok za donošenje odluke o kakvom se mogućem
kvarnom stanju sustava radi. Ako je sustav bez kvarnog stanja, tada
su dobivena odstupanja izmedju karakterističkih veličina jednake nuli.
Ako ta odstupanja nisu jednaka nuli nego prelaze odredjeni prag u sustavu
postoji kvarno stanje. Obično se odstupanja računaju s raznim kombinacijama
stvarnih i mjerenih veličina tako da se može izvršiti jednostavna
dijagnostika nastanka kvarnog stanja. Metoda je osjetljiva na smetnje
koje mogu nastati u sustavu. Zato se izračunana odstupanja moraju
dodatno procesirati da bi se utvrdio mogući nastanak kvarnog stanja,
što je prikazano načelnom shemom na na slici \ref{fig:ident_i_lok}

\begin{figure}
\begin{centering}
\includegraphics[scale=0.5]{chapters/Chapter5/figures/Rezidual.pdf}
\par\end{centering}
\caption{Načelna shema za identifikaciju i lokalizaciju kvarnih stanja kod
aktivnih metoda \cite{Kniga_paton_chen2012robust}. \label{fig:ident_i_lok}}

\end{figure}

Za potrebe generiranja reziduala (slika \ref{fig:ident_i_lok}) najčešće
se koriste metode zasnovane na modelu (matematičkom ili apriori) i
metode zasnovane na podacima (slika \ref{Dijagnoza kvara}). Nadalje,
metode koje se zasnivaju na matematičkom modelu (koje se koriste u
ovoj disertaciji) za dijagnosticiranje kvarnog stanja su:

\medskip{}
\begin{itemize}
\item \textbf{Estimacija stanja.} U ove metode potpadaju metode zasnovane
na obzerverima \cite{Obzerver_adjallah1994non}, \cite{SMC_obzerver_sreedhar1993robust}
i metode zasnovane na Kalmanovu filtru \cite{Obzerver_adjallah1994non},\cite{Kalman_II_chamseddine2015experimental}.
Metode zasnovane na obzerverima rekonstruiraju izlazi signal sustava
koji se dobiva na osnovi matematičkog modela sustava u slučaju rada
bez prisustva kvarnog stanja. Ovaj se obzerver općenito razlikuje
od obzervera koji se koristi za potrebe upravljanja. Za razliku od
obzervera za potrebe upravljanja, koji vrši estimaciju stanja koja
nisu neposredno mjerljiva, obzerver za dijagnozu kvarnih stanja vrši
estimaciju mjerenih varijabli sustava. Zatim se generira rezidual
na osnovu stvarnih i estimiranih vrijednosti mjerenih varijabli. 
\end{itemize}
\medskip{}
\begin{itemize}
\item \textbf{Parametarska identifikacija}. Parametarska identifikacija
oslanja se na pretpostavku da će u slučaju nastanka kvarnog stanja
u sustavu doći do odredjene promjene pojedinih parametara kao posljedice
nastanka kvarnog stanja. Parametarske metode mogu biti preciznije
i pouzdanije u odnosu na analitičke metode ali imaju veće zahtjeve
u smislu stvarno-vremenskog računanja \cite{gertler1998fault}. Kod
parametarske se identifikacije odredjuju nazivne vrijednosti svih parametara
u sustavu bez prisustva kvarnog stanja, te se iste koriste kao referentne
vrijednosti u slučaju nastanka kvarnog stanja. Rezidual se formira
izmedju estimiranih vrijednosti parametara koji se dobivaju iz mjerenih
podataka primjenom nekih od metoda identifikacije (metoda najmanjih
kvadrata (\emph{engl.} least squares), rekurzivna metoda najmanjih
kvadrata (\emph{engl.} recursive least squares) i proširena metoda
najmanjih kvadrata (\emph{engl.} extended least squares)) i nazivnih
vrijednosti parametara koje su inicijalno dobivene.
\end{itemize}
\medskip{}
\begin{itemize}
\item \textbf{Istovremena estimacija stanja i parametarska identifikacija}.
Za istovremenu estimaciju stanja i parametara sustava veoma je raširena
upotreba proširenog Kalmanova filtra (\emph{engl.} extended Kalman
filter - EKF) \cite{Kalman_EKF_amoozgar2013experimental} i višestupanjskog
Kalmanova filtra (\emph{engl.} Two-stage Kalman Filter). U radu \cite{ducard2008efficient}
opisano je korištenje proširenog Kalmanova filtra za identifikaciju
i lokalizaciju nastanka kvarnog stanja korištenjem banke proširenih
Kalmanovih filtara. Za generiranje reziduala korištenjem Kalmanova
filtra, isti se koristi za predikciju kvarnog stanja u sustavu, a
potom se usporedjuje kvarno stanje stvarnog sustava i predikcije dobivene
Kalmanovim filtrom. Ako je ta razlika jednaka nuli to indicira da
u sustavu nije nastalo kvarno stanje, a za slučaj da postoji odstupanje
iznad unaprijed definiranog praga tada je nastalo kvarno stanje. Matematički
je zapis Kalmanova filtra jednostavan, te je i njegova implementacija
relativno jednostavna. Medjutim, za svaku vrstu kvarnog stanja u sustavu
potrebno je projektirati po jedan filtar što može dovesti do toga
da imamo veliki broj filtara koje treba provjeriti da bi se pronašla
hipoteza koja odgovara trenutnom stanju u sustavu. U radu \cite{zhang2008bibliographical}
navodi se da najbolje sveukupne performanse imaju metode zasnovane
na simultanoj estimaciji stanja i parametara, s obzirom da nasljedjuju
prednosti ovih pojedinačnih metoda.
\end{itemize}
\medskip{}
\begin{itemize}
\item \textbf{Jednadžbe pariteta }(\emph{engl.} Parity space). Osnovna je
ideja ovoga pristupa da se eliminiraju nepoznata stanja, a potom se
dobivaju relacije u kojima su poznata sva stanja. Metode zasnovane
na paritetnom prostoru izvršavaju linearne dinamičke transformacije
veze izmedju ulaza i izlaza. Provjera pariteta obavlja se usporedbom
pariteta modela i mjerenja. Razlika koja se dobiva upotrebom transformacije
služi za otkrivanje i izolaciju kvarnog stanja. Izvodjenje relacija
za paritetni prostor zasnovan na prostoru stanja dano je u radu \cite{gertler1990new}.
\end{itemize}
\medskip{}

U sljedećem potpoglavlju prikazuje se jednostavni sustav za otkrivanje
i izolaciju kvarnih stanja u pogonskom sustavu zasnovan na metodi
najmanjih kvadrata \cite{Osmic_AIM}. Primarni razlog za odabir te
metode jest njezina jednostavna implementacija koja daje dobre performanse.

\newpage{}

\section{RLS-based fault-tolerant tracking control}


 \color{blue}


In order to exploit the results of the fault-dependent MAV maneuverability analysis, presented in Section 5. and to provide a unique testbed for performance analysis of considered motion planners, a mechanism for failure detection and fault-tolerant tracking control is needed. In this section, we briefly describe the approach we previously presented in \cite{Osmic_AIM}.

As shown in Chapter 2, the relation between the control inputs $u$ (the reference thrust  force $T$ and torques $\boldsymbol{\tau}$) and the rotation velocity $\boldsymbol{\Omega}_s$ of DC motors is given with $\boldsymbol{u_{ref}} = \boldsymbol{A} \boldsymbol{\Omega}_s$ (see Section 2.), where the control vector $\boldsymbol{u_{ref}}$ is represented by:





 

\begin{equation}
\boldsymbol{u_{ref}}=\begin{bmatrix}T & \boldsymbol{\tau}\end{bmatrix}^{T}=\begin{bmatrix}T & \tau_{x} & \tau_{y} & \tau_{z}\end{bmatrix}^{T},\label{eq:Upravljanje_za_FTC}
\end{equation}
$A$  being the system actuation matrix defined as (for PNPNPNPN configuration):

\begin{equation}
\boldsymbol{A}=\begin{bmatrix}b & b & b & b & b & b & b & b\\
bl & \frac{\sqrt{2}}{2}bl & 0 & -\frac{\sqrt{2}}{2}bl & -bl & -\frac{\sqrt{2}}{2}bl & 0 & \frac{\sqrt{2}}{2}bl\\
0 & -\frac{\sqrt{2}}{2}bl & -bl & -\frac{\sqrt{2}}{2}bl & 0 & \frac{\sqrt{2}}{2}bl & bl & \frac{\sqrt{2}}{2}bl\\
-d & d & -d & d & -d & d & -d & d
\end{bmatrix},\label{eq:Akt_PNPNPNPN}
\end{equation}
$\boldsymbol{\Omega}_{s}$ represents the squared rotor velocity vector
given as: 

\begin{equation}
\boldsymbol{\Omega}_{s}=\begin{bmatrix}\Omega_{1}^{2} & \Omega_{2}^{2} & \Omega_{3}^{2} & \Omega_{4}^{2} & \Omega_{5}^{2} & \Omega_{6}^{2} & \Omega_{7}^{2} & \Omega_{8}^{2}\end{bmatrix}^{T}.\label{eq:Vektor_kutnih_btzina}
\end{equation}

\color{black}

Članovi aktuacijske matrice $\boldsymbol{A}$ zavise samo od aerodinamičkih
karakteristika propelera i odabranog tipa letjelice. Shodno tome,
referentni upravljački signal letjelice izravno je proporcionalan
kvadratu kružnih brzina propelera $\omega_{i}$ ($i=\overline{1..8}$).
Za slučaj kvarnog stanja na nekom od pogonskih motora, pojedine komponente
referentnog upravljačkog signala se promijene. 


\color{blue}


To design fault-tolerant control, it is necessary to include information about faulty states of DC motors into the actuation matrix. In order to be able to take into account faulty states of DC motors, we will define the rotor capacity vector $\boldsymbol{\theta}$,
where $\boldsymbol{\theta} = \begin{bmatrix}
\theta_1 &\theta_2 &\theta_3 &\theta_4 &\theta_5 &\theta_6 &\theta_7 &\theta_8 \end{bmatrix}^T$ represents the faulty states of DC motors. The coefficients $0 \leq \theta_i \leq 1 \; (i = \overline{1..8})$ represent the failure level of related DC motor, where $\theta=1$ represents fully available motor, $\theta=0$ failed motor while all values in between represent a partial loss of DC motor functionality. Now we can rewrite the actuation matrix as:
\begin{equation}
\boldsymbol{u_{ref}} = \boldsymbol{A} \text{diag}\left(\boldsymbol{\Omega}_s\right)\boldsymbol{\theta},
\label{lin_model}
\end{equation}




If we individual rows of reference control vectors $\boldsymbol{A}$  define as:

\begin{equation}
\begin{array}{c}
\boldsymbol{A}_{T}=\begin{bmatrix}b & b & b & b & b & b & b & b\end{bmatrix}\\
\boldsymbol{A}_{1}=\begin{bmatrix}bl & \frac{\sqrt{2}}{2}bl & 0 & -\frac{\sqrt{2}}{2}bl & -bl & -\frac{\sqrt{2}}{2}bl & 0 & \frac{\sqrt{2}}{2}bl\end{bmatrix}\\
\boldsymbol{A}_{2}=\begin{bmatrix}0 & -\frac{\sqrt{2}}{2}bl & -bl & -\frac{\sqrt{2}}{2}bl & 0 & \frac{\sqrt{2}}{2}bl & bl & \frac{\sqrt{2}}{2}bl\end{bmatrix}\\
\boldsymbol{A}_{3}=\begin{bmatrix}-d & d & -d & d & -d & d & -d & d\end{bmatrix}
\end{array},\label{eq:A_parametrizacije}
\end{equation}
then actuation matrix can be represented in form:

\begin{equation}
A=\left[\begin{array}{cccc}
\boldsymbol{\boldsymbol{A^{T}}_{T}} & \boldsymbol{A^{T}}_{1} & \boldsymbol{A^{T}}_{2} & \boldsymbol{A^{T}}_{3}\end{array}\right]^{T}.\label{eq:A_vektorski}
\end{equation}

Then, the components of the $T$, $\boldsymbol{\tau_{x}}$, $\boldsymbol{\tau_{y}}$ and  $\boldsymbol{\tau_{z}}$ vectors of the controllable control signals $\boldsymbol{u}$ can be represented as weighted scalar products in the form :

 

\begin{equation}
\begin{array}{c}
T=\boldsymbol{A}_{T}\text{diag}\left(\boldsymbol{\Omega}_{s}\right)\boldsymbol{\theta}\\
\tau_{x}=\boldsymbol{A}_{1}\text{diag}\left(\boldsymbol{\Omega}_{s}\right)\boldsymbol{\theta}\\
\tau_{y}=\boldsymbol{A}_{2}\text{diag}\left(\boldsymbol{\Omega}_{s}\right)\boldsymbol{\theta}\\
\tau_{z}=\boldsymbol{A}_{3}\text{diag}\left(\boldsymbol{\Omega}_{s}\right)\boldsymbol{\theta}.
\end{array},\label{eq:pojedinacne_komponente}
\end{equation}




As we can see from \eqref{eq:pojedinacne_komponente}, the control output can be represented by its four components that have a linear dependence. Based on these values, it is possible to estimate the parameter $\boldsymbol{\theta}$ in a least-squares manner. For the estimation, it is necessary to know all parameters in \eqref{eq:pojedinacne_komponente}. The basic requirement is that the values of the actuation matrix $\boldsymbol {A}$ are a priori known. For the detection and isolation of failures, we only use gyroscopic data for their inherent accuracy of measurement so that the first equality from \eqref{eq:pojedinacne_komponente} is not necessary, so the final prediction is:

\[
\begin{array}{c}
\tau_{x}=\boldsymbol{A}_{1}\text{diag}\left(\boldsymbol{\Omega}_{s}\right)\boldsymbol{\theta}\\
\tau_{y}=\boldsymbol{A}_{2}\text{diag}\left(\boldsymbol{\Omega}_{s}\right)\boldsymbol{\theta}\\
\tau_{z}=\boldsymbol{A}_{3}\text{diag}\left(\boldsymbol{\Omega}_{s}\right)\boldsymbol{\theta}.
\end{array}
\]

\color{black}

Za predikciju izlaza $\tau_{x}$,$\tau_{y}$ i $\tau_{z}$ potrebne
su i prethodne vrijednosti, pa se koristi dinamički model kružnog
gibanja sustava oktokoptera dan s:

\begin{equation}
\begin{array}{c}
\dot{P}=\frac{I_{yy}-I_{zz}}{I_{xx}}QR+\frac{\tau_{x}}{I_{xx}}-\frac{I_{zzm}}{I_{xx}}W_{g}Q\\
\dot{Q}=\frac{I_{zz}-I_{xx}}{I_{yy}}PR+\frac{\tau_{y}}{I_{yy}}+\frac{I_{zzm}}{I_{yy}}W_{g}P\\
\dot{R}=\frac{I_{xx}-I_{yy}}{I_{zz}}PQ+\frac{\tau_{z}}{I_{zz}}.
\end{array}\label{eq:dinamicki_model_octo}
\end{equation}
Korištenjem veze izmedju $\tau_{x}$,$\tau_{y}$ i $\tau_{z}$ i dinamičkog
modela oktokoptera danu s \ref{eq:dinamicki_model_octo}, povijest
potrebnih izlaza $\tau_{x}$,$\tau_{y}$ i $\tau_{z}$ možemo rekonstruisati
kao :

\begin{equation}
\begin{array}{c}
\tau_{x}=I_{xx}\dot{P}-(I_{yy}-I_{zz})QR+I_{zzm}W_{g}Q\\
\tau_{y}=I_{yy}\dot{Q}-(I_{zz}-I_{xx})PR-I_{zzm}W_{g}P\\
\tau_{z}=I_{zz}\dot{R}-(I_{xx}-I_{yy})PQ.
\end{array}\label{eq:histroija_izlaza}
\end{equation}
Iz jednadžbe \ref{eq:histroija_izlaza} može se uočiti da je za rekonstrukciju
izlaza $\tau_{x}$,$\tau_{y}$ i $\tau_{z}$ neophodno poznavati članove:
$I_{xx}$, $I_{yy}$ i $I_{zz}$ tenzora inercije letjelice, vrijednosti
kružnih ubrzanja $\dot{P}$, $\dot{Q}$ i $\dot{R}$, moment inercije
rotora $I_{zzm}$ i žiroskopsku komponentu $W_{g}$. Iz očitanja žiroskopa
dostupne su nam vrijednosti kružne brzine $P$, $Q$ i $R$. Na osnovi
tih vrijednosti, kružna ubrzanja $\dot{P}$, $\dot{Q}$ i $\dot{R}$
mogu se dobiti numeričkim diferenciranjem kružnih brzina $P$, $Q$
i $R$. Žiroskopska komponenta $W_{g}$ dobiva se izravnim izračunom
iz mjerenja kružnih brzina vrtnje rotora. Da bismo dobili uvid u predloženu
metodu, razmotrit ćemo slučaj da se otkrivanje i izolacija kvarnog
stanja obavlja samo na osnovi jedne od vrijednosti $\tau_{x}$,$\tau_{y}$
i $\tau_{z}$ . Prvo razmotrimo slučaj da predikciju vršimo samo na
osnovi vrijednosti $\tau_{x}$. Tada je

\begin{equation}
\tau_{x}=\left[\begin{array}{cccc}
\tau_{x}(1) & \tau_{x}(2) & \cdots & \tau_{x}(N)\end{array}\right]^{T}.\label{eq:predikcija_Y1}
\end{equation}
Za ovaj su slučaj regresori oblika:

\begin{equation}
\begin{array}{c}
\boldsymbol{\psi}_{1}(1)=\boldsymbol{A}_{1}\text{diag}\left(\boldsymbol{\Omega}_{s}(1)\right)\\
\boldsymbol{\psi}_{1}(2)=\boldsymbol{A}_{1}\text{diag}\left(\boldsymbol{\Omega}_{s}(2)\right)\\
\vdots\\
\boldsymbol{\psi}_{1}(N)=\boldsymbol{A}_{1}\text{diag}\left(\boldsymbol{\Omega}_{s}(N)\right)
\end{array},\label{eq:regeresori_Y1}
\end{equation}
dok matrica podataka ima oblik:

\begin{equation}
\boldsymbol{\Psi}_{1}=\left[\begin{array}{cccc}
\boldsymbol{\Psi}_{1}(1) & \boldsymbol{\Psi}_{1}(2) & \cdots & \boldsymbol{\Psi}_{1}(N)\end{array}\right]^{T}.\label{eq:matrica_podataka_Y1}
\end{equation}
Razmotrimo slučaj da predikciju vršimo samo na osnovi vrijednosti
$\tau_{y}$. U ovom slučaju imamo:

\begin{equation}
\tau_{y}=\left[\begin{array}{cccc}
\tau_{y}(1) & \tau_{y}(2) & \cdots & \tau_{y}(N)\end{array}\right]^{T}.\label{eq:predikcija_Y2}
\end{equation}
Za ovaj su slučaj regresori oblika:

\[
\begin{array}{c}
\boldsymbol{\psi}_{2}(1)=\boldsymbol{A}_{2}\text{diag}\left(\boldsymbol{\Omega}_{s}(1)\right)\\
\boldsymbol{\psi}_{2}(2)=\boldsymbol{A}_{2}\text{diag}\left(\boldsymbol{\Omega}_{s}(2)\right)\\
\vdots\\
\boldsymbol{\psi}_{2}(N)=\boldsymbol{A}_{2}\text{diag}\left(\boldsymbol{\Omega}_{s}(N)\right)
\end{array},
\]
dok matrica podataka poprima oblik:

\begin{equation}
\boldsymbol{\Psi}_{2}=\left[\begin{array}{cccc}
\boldsymbol{\Psi}_{2}(1) & \boldsymbol{\Psi}_{2}(2) & \cdots & \boldsymbol{\Psi}_{2}(N)\end{array}\right]^{T}.\label{eq:matrica_podataka_Y2}
\end{equation}
Konačno, ako se za predikciju koristi samo vrijednost $\tau_{z}$
tada je vektor izlaza dan kao: 


\begin{equation}
\tau_{z}=\left[\begin{array}{cccc}
\tau_{z}(1) & \tau_{z}(2) & \cdots & \tau_{z}(N)\end{array}\right]^{T}\label{eq:predikcija_Y3}
\end{equation}
{dok su regresori oblika:}


\[
\begin{array}{c}
\boldsymbol{\psi}_{3}(1)=\boldsymbol{A}_{3}\text{diag}\left(\boldsymbol{\Omega}_{s}(1)\right)\\
\boldsymbol{\psi}_{3}(2)=\boldsymbol{A}_{3}\text{diag}\left(\boldsymbol{\Omega}_{s}(2)\right)\\
\vdots\\
\boldsymbol{\psi}_{3}(N)=\boldsymbol{A}_{3}\text{diag}\left(\boldsymbol{\Omega}_{s}(N)\right)
\end{array},
\]
a matrica podataka je oblika:

\begin{equation}
\boldsymbol{\Psi}_{3}=\left[\begin{array}{cccc}
\boldsymbol{\Psi}_{3}(1) & \boldsymbol{\Psi}_{3}(2) & \cdots & \boldsymbol{\Psi}_{3}(N)\end{array}\right]^{T}.\label{eq:matrica_podataka_Y3}
\end{equation}

\medskip{}
Razmotrimo poziciju oktokoptera u odnosu na globalni i lokalni koordinatni
sustav predstavljen slikom \ref{fig:globalni_i_lokalni_koor_sistem}
kao i matricu aktuacije danu s \ref{eq:Akt_PNPNPNPN}. Iz slike \ref{fig:globalni_i_lokalni_koor_sistem}
i jednadžbe \ref{eq:Akt_PNPNPNPN} može se uočiti da parametri $\theta_{3}$
i $\theta_{7}$ vektora kapaciteta rotora nemaju utjecaja na formiranje
izlaza $\tau_{x},$ a isto tako parametri $\theta_{1}$ i $\theta_{5}$
vektora kapaciteta rotora nemaju utjecaj na formiranje izlaza $\tau_{y}$.
To praktički znači da se komponente $\theta_{3}$ i $\theta_{7}$
vektora kapaciteta rotora ne mogu odrediti iz izlaza $\tau_{x}$,
a isto tako ni komponente $\theta_{1}$ i $\theta_{5}$ vektora kapaciteta
rotora ne mogu se odrediti iz izlaza $\tau_{y}$. Nasuprot tome svi
parametri vektora kapaciteta rotora imaju utjecaj na formiranje izlaza
$\tau_{z}$. Kako bi se poboljšala točnost iskoristit ćemo sve izlaze
koji su nam na raspolaganju ($\tau_{x}$,$\tau_{y}$ i $\tau_{z}$)
za odredjivanje predikcije pojedinih komponenata vektora kapaciteta
rotora, pa vektor izlaza možemo zapisati u obliku:

\begin{figure}
\begin{centering}
\includegraphics[scale=0.5]{chapters/Chapter5/figures/Frame.pdf}
\par\end{centering}
\caption{Body and ground fixed frames.\label{fig:globalni_i_lokalni_koor_sistem}}

\end{figure}

\begin{equation}
\boldsymbol{\tau}=\left[\begin{array}{cccccccccc}
\tau_{x}(1) & \tau_{y}(1) & \tau_{z}(1) & \tau_{x}(2) & \tau_{y}(2) & \tau_{z}(2) & \cdots & \tau_{x}(N) & \tau_{y}(N) & \tau_{z}(N)\end{array}\right]^{T}.\label{eq:predikcija_izlaza_full}
\end{equation}
Za ovaj su slučaj regresori oblika:

\begin{equation}
\Psi=\left[\begin{array}{cccccccccc}
\psi_{1}^{T}(1) & \psi_{2}^{T}(1) & \psi_{3}^{T}(1) & \psi_{1}^{T}(2) & \psi_{2}^{T}(2) & \psi_{3}^{T}(2) & \cdots & \psi_{1}^{T}(N) & \psi_{2}^{T}(N) & \psi_{3}^{T}(N)\end{array}\right]^{T},\label{eq:Regresori_full}
\end{equation}
i matrica podataka:

\begin{equation}
\boldsymbol{\Psi}=\left[\begin{array}{cccc}
\boldsymbol{\psi}(1) & \boldsymbol{\psi}(2) & \cdots & \boldsymbol{\psi}(3N)\end{array}\right]^{T}.\label{eq:predikcija_konacna}
\end{equation}
Vrijednosti regresora dobiveni s (\ref{eq:predikcija_konacna}) mogu
se koristiti za odredjivanje parametara vektora kapaciteta rotora korištenjem
rekurzivnog oblika metode najmanjih kvadrata koja se zasniva na ne-rekurzivnoj
jednadžbi metode najmanjih kvadrata \cite{isermann_ident}):

\[
\boldsymbol{\theta}=\left(\boldsymbol{\Psi}^{T}\boldsymbol{\Psi}\right)^{-1}\boldsymbol{\Psi}^{T}\boldsymbol{\tau}.
\]

Vrijednosti za $\ensuremath{\ensuremath{\ensuremath{\theta_{i}\;(i=\overline{1..8})}}}$,
nisu konstantne cijelo vrijeme, pa je korišten faktor zaboravljanja
da bi se predložena tehnika mogla primijeniti na višerotorski sustav.
Neophodno je naglasiti da se predložena tehnika, zasnovana na metodi
najmanjih kvadrata, za procjenu vrijednosti kapaciteta vektora rotora
može primijeniti na bilo kojoj višerotorskoj letjelici s $n$ pari
rotora u planarnoj konfiguraciji. Kako bismo mogli iskoristiti informaciju
o kapacitetu rotora odnosno o kvarnom stanju, u sljedećem potpoglavlju
predstavljamo upravljačku arhitekturu koja može iskoristiti informaciju
o procjeni vrijednosti kapaciteta vektora rotora bespilotne višerotorske
letjelice.

\subsection{Simulation results for fault-tolerant PD
tracking control }



U 3. poglavlju opisana je procedura projektiranja regulatora za praćenje
referentne trajektorije. Kako bismo mogli iskoristiti informaciju
o identifikaciji nastanaka kvarnog stanja (lokacija i intenzitet kvarnog
stanja) proširit ćemo predloženu arhitekturu na način kako je to pokazano
na slici \ref{fig:FTC_arhitektura}.

\begin{figure}
\begin{centering}
\includegraphics[scale=0.5]{chapters/Chapter5/figures/FTC_arhitektura.pdf}
\par\end{centering}
\caption{Fault-tolerant PD tracking control architecture\label{fig:FTC_arhitektura}\cite{Osmic_AIM}.}

\end{figure}

Kako se može uočiti sa slike \ref{fig:FTC_arhitektura}, na ulaze
regulatora pozicije, visine i zakreta dovode se referentne vrijednosti
za poziciju $x$, $y$ i $z$ koordinatu u prostoru i referenca za
orijentaciju $\psi$ (njihove vrijednosti uobičajeno generira planer
gibanja). Regulatori pozicije, visine i zakreta na svojim izlazima
generiraju potrebnu referentnu silu potiska i momente kako bi se referentne
koordinate za poziciju i zakret dosegle, odnosno vektor upravljačke
varijable ima oblik:

\begin{equation}
\boldsymbol{u_{ref}}=\begin{bmatrix}T & \boldsymbol{\tau}\end{bmatrix}^{T}=\begin{bmatrix}T & \tau_{x} & \tau_{y} & \tau_{z}\end{bmatrix}^{T}=\boldsymbol{A}\boldsymbol{\Omega}_{s},\label{eq:alokacija_upr}
\end{equation}

Referentno upravljanje postiže se pomoću pogonskih motora, odnosno
tako da se pogonski motori vrte na način da generirana sila bude što
bliža referentnoj. Za slučaj kada matrica aktuacije ima kvadratnu
formu, zadatak se svodi na pronalaženje inverzije matrice $A,$ pa
se potrebne brzine pogonskih motora računaju kao $\ensuremath{\boldsymbol{\Omega_{s}}=\boldsymbol{A}^{-1}\boldsymbol{u_{ref}}}$.
Medjutim, kako je već ranije naglašeno, budući da se ovdje radi o sustavu
višerotorske letjelice s $2n$ pari motora (oktokopter s $n=4)$,
to imamo više pogonskih motora nego je to neophodno, pa se referentne
vrijednosti upravljačke varijable mogu realizirati na beskonačno mnogo
načina. Kako matrica aktuacije, za slučaj oktokoptera, nema kvadratnu
formu to se ne može koristiti prosta inverzija za proračun potrebnih
brzina motora koji osiguravaju referentne vrijednosti upravljačke
varijable. Jedan je od često korištenih načina postizanja referentnog
upravljanja korištenje upravljačke alokacije tako da se za izračun
referentnog vektora upravljanja iskoristi pseudo-inverzija \cite{basson_pseudo,FTC_ETH_Thomas_Schneider}.
Za navedeni slučaj (gdje matrica aktuacije nema kvadratnu formu) proračun
referentnog upravljanja se računa po formuli:

\begin{equation}
\boldsymbol{\Omega_{s}}=\boldsymbol{A}^{+}\boldsymbol{u_{ref}}\label{eq:pseudo_osnovna}
\end{equation}
gdje je {$\boldsymbol{A}^{+}=\boldsymbol{A}^{T}(\boldsymbol{A\boldsymbol{A}^{T}})^{-1}$.}


\medskip{}


Proračun referentnog upravljanja korištenjem pseudo-inverzije osigurava
barem jednu od mogućih kombinacija pomoću koje se doseže referentno
upravljanje. Medjutim, za slučaj kvarnog stanja, jedan ili više pogonskih
motora neće imati nikakav doprinos u matrici aktuacije pa će proračun
pomoću pseudo-inverzije dati netočno rješenje. U prethodnom smo potpoglavlju
pokazali da se korištenjem metode zasnovane na metodi najmanjih kvadrata
mogu odrediti kapaciteti vektora rotora. Kako su nam kapaciteti vektora
rotora dostupni, te uzimajući u obzir činjenicu da su vektori {$\Omega_{s}$
i $\theta$ vektori iste veličine, }jednadžba (\ref{eq:alokacija_upr})
može se zapisati u obliku:

\begin{equation}
\boldsymbol{u_{ref}}=\boldsymbol{A}\text{diag}\left(\boldsymbol{\theta}\right)\boldsymbol{\boldsymbol{\Omega}_{s}}.\label{eq:kapaciteti_konacna}
\end{equation}

\color{blue}


Furthermore, by introducing a new matrix $\boldsymbol{B}$ as $\boldsymbol{B} = \boldsymbol{A} \text{diag}\left(\boldsymbol{\theta}\right)$, we can calculate the velocity for all DC motors that can achieve the reference thrust and the torques as
\begin{equation}
\label{pseudo_konacana}
\boldsymbol{\Omega_s}= \boldsymbol{B}^{+}\boldsymbol{u_{ref}},
\end{equation}

where $\boldsymbol{B}^{+}=\boldsymbol{B}^{T}(\boldsymbol{B\boldsymbol{B}^{T}})^{-1}$.




\color{blue}


For ilustration purpose, we present the simulation results for the RLS-based technique for detection and isolation  of DC motor failures on MAVs. We used a fault-tolerant PD tracking control system around the hovering configuration. To illustrate that the designed controller can handle a faulty state on MAV,  we consider octocopter with the PNPNPNPN conﬁguration. In this case, we have a failure occured on the 3rd motor at time $t=5$ $[s]$. This case can be expressed by the rotor capacity vector $\boldsymbol{\theta} = \begin{bmatrix} 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1\end{bmatrix}^T$.


It should be emphasized that the presented approach was tested for different classes of possible faults (different numbers of faulty rotors and different values of rotor capacity). For the purpose of the RLS algorithm, we need to determine 8 unknowns parameters $\theta_{i}$, so we need at least 8 equations. It follows, that the number of samples $N$ must be at least $N\geq8$.  However, to eliminate the impact of noise, it is advisable to use a larger number of equations, that is $N\gg8$. So, we set the forgetting factor to 0.8 in order to take into account the measurements from the previous 0.8 seconds to provide a sufficient number of samples for the RLS algorithm.

Figs. \ref{fig:Vivijani_pracenje_3D_M3} and \ref{fig:Vivijani_pogreska_M3} depict the performance of the proposed RLS-based PD tracking controller with control allocation for a failure occured on the 3rd motor  at $t=5$ $[s]$. Fig. \ref{fig:Vivijani_parametri_M3} shows that the relative capacity of each rotor is properly diagnosed. \color{black}  Na slici \ref{fig:Vivijani_parametri_M3} plavom bojom su prikazani stvarni kapaciteti pogonskih motora a crvenom bojom estimirani. Sa slike se može uočiti da predložena metoda dobro
estimira parametre.  

 \color{blue}

From Fig.\ref{fig:Vivijani_pogreska_M3}, we can conclude that the presented RLS controller has an acceptable tracking performance (it is similar to the tracking performance for a healthy MAV). This can be attributed to the inherent fault-tolerability of the octocopter platform, as can be expected based on the analysis of fault-dependent maneuverability for octocopter provided in Section 5.). 
\color{black}



\begin{figure}
\begin{centering}
\includegraphics[scale=0.9]{chapters/Chapter5/figures/3D_fault_M3.pdf}
\par\end{centering}
\caption{3D visualization of tracking performance (an octocopter with the PNPNPNPN conﬁguration) for a failure occured on the 3rd motor at $t=5$ $[s]$.\label{fig:Vivijani_pracenje_3D_M3}}
\end{figure}

\begin{figure}
\begin{centering}
\includegraphics[scale=0.9]{chapters/Chapter5/figures/Pracenje_fault_M3.pdf}
\caption{Left: reference values, Right: tracking error for a failure occured on the 3rd motor at $t=5$ $[s]$.}.\label{fig:Vivijani_pogreska_M3}
\par\end{centering}
\end{figure}

\begin{figure}
\begin{centering}
\includegraphics[scale=0.9]{chapters/Chapter5/figures/Parametri_fault_M3.pdf}
\par\end{centering}
\caption{Estimation of relative capacity of each rotor during
the tracking task for fault state (DC motor 3 for $t\geqslant5$) blue: real capacity of rotor, red: estimated capacity of rotor.
\label{fig:Vivijani_parametri_M3}}

\end{figure}

==> chapters/Chapter6/ch6.tex <==
\chapter{\medskip{}
{Analiza utjecaja kvarnih stanja i njihova
djelovanja na bespilotnu letjelicu} \label{chap:FTC}}


Analiza utjecaja kvarnih stanja i njihovih djelovanja (u daljnjem
tekstu FMEA:{\emph{engl.}}- \textbf{F}ailure
\textbf{M}ode and\textbf{ E}ffects \textbf{A}nalysis) na bespilotnu
letjelicu s električnim pogonskim motorima, koja će biti predstavljena
u ovom poglavlju, razmatra osjetljivost sustava na kvarna stanja tijekom
normalnog izvršavanja operacija. Glavni je cilj analize razumjeti
uzrok i ozbiljnost kvarnih stanja koja mogu nastati na bespilotnoj
letjelici. Bespilotne letjelice obavljaju raznovrsne tipove zadataka
i može se dogoditi da uslijed nastanka kvarnog stanja bespilotna letjelica
ne može na željeni način ispuniti odredjeni zadatak. Iz toga je razloga
potrebna FME analiza, da bi se primjerenim održavanjem, pogodnim projektiranjem
upravljanja i pogodnim planiranjem misije, pripremilo letjelicu za
eventualne akcije koje treba poduzeti u slučaju nastanka kvarnog stanja.
Znajući vjerojatnost nastanka i ozbiljnost mogućeg kvarnog stanja,
moguće je procijeniti rizik nastalog kvarnog stanja po ukupni integritet
letjelice i planirane misije s kojim se sustav suočava tijekom misije.


\section{Uvodna razmatranja o projektiranju letjelica i FME analizi}

\color{green}

 During the process of UAV design, there are few aspects that should be discussed \cite{torun2000uav}. Two most important aspects in early stages of development were endurance and range. Today these aspects include load, safety and funcionality \cite{elands2016technical}. Safety is usually achieved through hardware redudancy and some other methods such as adaptive control and early fault detection \cite{FTC_ETH_Thomas_Schneider}, \cite{freeman_2014}. 
 
 Functionality is achieved through selection of appropriate hardware and software modules. However, UAV design is complex assignment and has to be carried out by experts from different areas of expertise \cite{Dronovi_regulativa}. One of the most important necessities in design and development of UAVs is to have all requirements known in advance. 








\color{black}






U početcima je najveću zainteresiranost za ovu problematiku pokazala
vojna industrija \cite{Istorija_UAV_blom2010} koja je bila pokretač
istraživanja i najveći financijer razvoja bespilotnih letjelica. Suradnja
vojne i zrakoplovne industrije, kao i akademske zajednice pokrenula
je ubrzan razvoj bespilotnih letjelica, tako da danas u svijetu postoji
veliki broj bespilotnih letjelica (zrakoplovi i helikopteri), koje
obavljaju raznovrsne zadatke, kako za potrebe vojske tako i za civilne
svrhe.{ Prve bespilotne letjelice koje su
se pojavile početkom devedesetih godina dvadesetog stoljeća, zasnivale
su se na konceptu klasičnih letjelica poput helikoptera, da bi se
kasnije prešlo na letjelice s fiksnim krilom, a u proteklom je desetljeću
došlo do intenzivnog razvoja višerotorskih letjelica. Najčešći izazov
kod projektiranja bespilotnih letjelica u civilnom sektoru predstavljaju
ograničena financijska sredstva \cite{bendea2008low}, \cite{neitzel2011mobile}.
Medjutim, u protekla dva desetljeća došlo je do intenzivne minijaturizacije
u području senzora i povećanja procesorske snage mikroračunala te
razvoja pouzdanijeg softvera, što je dovelo do toga da projektanti
bespilotnih letjelica ipak mogu u okviru predvidjenog budžeta razvijati
letjelice s pouzdanim komponentama za obavljanje zadataka za koje
su projektirane. Na tržištu trenutno dominiraju dvije vrste bespilotnih
letjelica: (i) letjelice s fiksnim krilima i (ii) višerotorske letjelice.}

\color{green}

When vehicle is designed it is important to investigate  possible situations that can occur during the UAV operations. There are various methods that are used for this type of analysis and investigation. 




One of the frequently used methods, conducted even in the conceptual stage of the system design, is failure mode and effects analysis (FMEA). This method is used to predict and handle different modes of failures effective and it turned out to be a really effective and reliable system engineering tool.

Even though the FMEA identifies and classifies all possible hazards in a system, the results of this analysis may not be comprehensive and has its limitations \cite{potts2014_FTC}. In addition, since the risk priority number (RPN), which is the measure used within the FMEA method, is based on different factors including failure severity, failure occurence frequency and failure detectability, some less serious failures might have higher RPN indications than some other more serious failures \cite{kmenta2004_ftc}. The ordinal rankings used to quantify the factors for all failure modes within the FMEA, only provide  the information that that one of the failure modes is higher ranked in terms of its criticality but it does not provide the exact information on what would be the difference between the RPN values of the two successive failure modes. For instance, a ranking of "4" may not be twice as severe as a ranking of "2".

\color{black}

 Ova vrijednost može biti
rezultat toga da je frekvencija pojavljivanja prvog kvarnog stanja
veća od frekvencije pojavljivanja drugog kvarnog stanja, ali da je
ozbiljnost po sustav manja ili ista. Zaključno, i pored toga što FME
analiza identificira i klasificira sva moguća kvarna stanja u sustavu,
rezultati analize nisu sveobuhvatni i imaju svoja ograničenja\cite{potts2014_FTC}.


\section{Osnove {analize utjecaja kvarnih stanja
i njihovih djelovanja na razmatrani sustav}}




\color{green}

Basically, there are two procedures or tools for system reliability and failure modes analysis: first one is inductive (bottom-up) and second is deductive (top-down). The FMEA can be used as bottom-up methodology used to discover and analyse possible system failure modes and effects of those failure modes on system or its parts and also to determine  their criticality. The FMEA is often limited to systems hardware components failures and consequences of those failures on system functionality. This procedure can be shortly explained as follows. All system components, their function and operation modes must be analysed and documented before proceeding with FMEA \cite{army2006failure}. Then, we analyse all failure modes that can occur during the operation of each component. After that, we analyse the effect of each failure mode of particular component,  to any other part of system and the system itself. A qualitative severity (or criticality) ranking is assigned to each potential failure and corresponding effect according to its potential damage and/or probability of occurrence. Doing the research and development stage several different severity criteria are formed. Resulting FMEA tables can serve as feedback to the design process, enabling revisions in early stages of development.




\color{black}


 
Svakom potencijalnom kvarnom stanju i njegovu mogućem učinku dodjeljuje
se kvalitativni stupanj ozbiljnosti (ili kritičnosti), s obzirom na
njegovu potencijalnu štetu i/ili vjerojatnost nastanka. U fazi istraživanja
i razvoja letjlelice razmatra se nekoliko različitih utjecaja koje
kvarna stanja mogu imati na sustav te se potom iz toga formira broj
$RPN$. Rezultati FMEA tablica mogu poslužiti kao povratna informacija
u procesu projektiranja, omogućujući izmjene u ranim fazama razvoja.



 \color{green}

One way in which failure modes are qualitatively classiﬁed \color{black}(dobivanje $RPN$ broja) \color{green}  is based on the following parameters \cite{freeman_2014}: 







Jedan od načina na koji su kvarna stanja kvalitativno razvrstana (dobivanje
$RPN$ broja) zasniva se na sljedećim parametrima \cite{freeman_2014}: 

\medskip{}
\begin{itemize}
\item likelihood of occurrence,
\item criticality of effects of that failure and
\item the overall risk for the system based on occurence and criticality. 
\end{itemize}
\medskip{}

Likelihood of failure modes for each system is not always possible to determine. Because of this, today we use rating scales to determine the criticality of failure. Criticality might be evaluated on a three-point scale which is very simple and consists of the following estimate factors: 

\medskip{}
\begin{itemize}
\item low (L),
\item medium (M) and
\item high (H). 
\end{itemize}
\medskip{}




\color{black} Pored opisanih kategorizacija, za ozbiljnost nastanka kvarnog stanja
često je u uporabi kategorizacija zasnovana na NASA-inim standardima
za FME analizu za letjelice{ \cite{NASA}}.

\color{green} Categories for criticality classification based on NASA standards for FMEA for vehicles were defined as follows:


\medskip{}

\begin{itemize}
\item \textbf{Category 1} - Catastrophic - Failure modes that could result in damage to the vehicle, property damage, serious injury, or loss of life,
\item \textbf{Category 1R} - 1R Catastrophic - Modes of identical or equivalent redundant hardware items that, if all failed, could result in Category 1 effects, 
\item \textbf{Category 2} - Critical - Failure modes that could result in loss of one or more mission objectives,
\item \textbf{Category 2R} - 2R Critical - Failure modes of identical or equivalent redundant hardware items that could result in Category 2 effects if all failed, 
\item \textbf{Category 3} - Significant - Failure modes that could cause serious errors in mission objectives and
\item \textbf{Category 4} -  Minor - Failure modes that could result in insignificant or no loss to mission objectives. 
\end{itemize}

\medskip{}



Possibility of failure and the criticality of its potential effects can be combined to provide a qualitative estimate of the risk. 

Scale with low (L), medium (M), and high (H) ratings is used to identify system weaknesses and prioritize future development and improvements of the UAV design and operations modes. One way to create risk matrix with low, medium and high risk from NASA standards for FMEA is shown in Table \ref{tab:FMEA-Risk-Matrix}. For example, if we have criticality with number 1, but with likelihood rating low then it has a rating medium (M) in three point scale mentioned earlier. 
Another way to approach and analyse this problem is numerical definition of parameters of system parts failure modes via:   


\begin{table}[H]
\caption{{FMEA RISK MATRIX \cite{freeman_2014}.\label{tab:FMEA-Risk-Matrix}{ }}}

\begin{center} { \small
  \begin{tabular}{|l|c|c|c|c|c|c|} \hline            & \multicolumn{6}{c|}{Criticality} \\ \hline Likelihood & 4   & 3   & 2R   & 2  & 1R  & 1  \\ \hline High       & \cellcolor[HTML]{F56B00}M   &  \cellcolor[HTML]{F56B00}M   & \cellcolor[HTML]{FE0000}H    & \cellcolor[HTML]{FE0000}H  & \cellcolor[HTML]{FE0000}H   & \cellcolor[HTML]{FE0000}H  \\ \hline  Medium     & \cellcolor[HTML]{34FF34}L   & \cellcolor[HTML]{F56B00}M   & \cellcolor[HTML]{F56B00}M    & \cellcolor[HTML]{F56B00}M   & \cellcolor[HTML]{FE0000}H   & \cellcolor[HTML]{FE0000}H  \\ \hline Low        & \cellcolor[HTML]{34FF34}L   & \cellcolor[HTML]{34FF34}L   & \cellcolor[HTML]{F56B00}M    & \cellcolor[HTML]{F56B00}M  & \cellcolor[HTML]{F56B00}M   & \cellcolor[HTML]{F56B00}M  \\ \hline \end{tabular}    } \end{center}
\end{table}


\medskip{}
\begin{itemize}
\item severity of faulty state,
\item occurrence of faulty state and 
\item detection of faulty state.
\end{itemize}
and finding of RPN number.  This approach is explained in detail in  \cite{FTC_ETH_Thomas_Schneider} for UAV with DC motors and \cite{osmic_FMEA} for a gasoline-powered UAV.

For a quantitative description of the fault state, this approach uses a total of three values are assigned in a range of 1-5: 

 \medskip{}
\begin{itemize}
\item occurrence (O in Table \ref{table_II})),
\item severity (S in Table \ref{table_II}) and 
\item detection (D in Table \ref{table_II}).
\end{itemize}
\medskip{}




\begin{table}[!b]
\caption{Rating for occurrence (O), severity (S) and detection(D)}
\label{table_II}
\begin{center}


{ \small
\begin{tabular} {|l|c|c|c|l|c|}
\hline
\multicolumn{6}{|c|}{FMEA Ratings}                                                                                                                                                                                                                                \\ \hline
     & O                                                    & S                                                    & D                                                        & \multicolumn{2}{l|}{RPN=O$\cdot$S$\cdot$D}                                                             \\ \hline
Rate & \multicolumn{3}{c|}{Description}                                                                                                                                       & \multicolumn{1}{c|}{value} &   effect                                                     \\ \hline
1    & Never                                                & \begin{tabular}[c]{@{}c@{}}No \\ effect\end{tabular} & \begin{tabular}[c]{@{}c@{}}Almost\\ certain\end{tabular} & \multicolumn{1}{c|}{1}   & No risk                                                \\ \hline
2    & Low                                                  & Minor                                                & High                                                     & $\leq$16             & \begin{tabular}[c]{@{}c@{}}Small \\ risk\end{tabular}  \\ \hline
3    & Medium                                               & Medium                                               & Medium                                                   & $\leq$30             & \begin{tabular}[c]{@{}c@{}}Medium \\ risk\end{tabular} \\ \hline
4    & High                                                 & High                                                 & Low                                                      & $\leq$125           & \begin{tabular}[c]{@{}c@{}}High\\  risk\end{tabular}   \\ \hline
5    & \begin{tabular}[c]{@{}c@{}}Very \\ high\end{tabular} & \begin{tabular}[c]{@{}c@{}}Very \\ high\end{tabular} & \begin{tabular}[c]{@{}c@{}}Very \\ remote\end{tabular}   &                          & \multicolumn{1}{l|}{}                                  \\ \hline
\end{tabular}
}
\end{center}
\end{table}




     
\medskip{}



\textbf{\textit{Occurrence of fault state (O)}} is divided in five categories

\medskip{}
\begin{itemize}
\item \textit{Never (1) }- so unlikely that it is not expected to happen in the entire lifetime of a system, 
\item \textit{Low (2)} - not expected to happen several times in the entire lifetime of the system,
\item \textit{Moderate (3)} - unlike to occur to all system during its lifetime or occur several times in lifetime,
\item \textit{High (4)} - occur most of the times and 
\item \textit{Very high (5)} - occurs all the times.
\end{itemize}
\medskip{}
\textbf{\textit{Severity of faulty state (S)}} is also divided into five categories:

\medskip{}
\begin{itemize}
\item \textit{No effect (1) - } has no effect on the system,
\item \textit{Minor (2)} - affects small part of the system noticed by average customers,
\item \textit{Moderate (3)} - most customers are annoyed,
\item \textit{High (4)} - caused a loss of primary function and customers are not satisfied and
\item \textit{Very high and hazardous} - product becomes inoperative.
\end{itemize}
\medskip{}
\textbf{\textit{Detection of faulty state (D)}} is also divided in five categories:

\medskip{}
\color{black}
\begin{itemize}
\item \textit{Almost certain (1)} - nastanak kvarnog stanje moguće je gotovo
uvijek otkriti,
\item \textit{High} (2) - kvarno stanje moguće je otkriti u velikom broju
slučajeva nastanka, 
\item \textit{Moderate} (3) - moguće otkrivanje odredjenog broja kvarnih stanja,
\item \textit{Low (4)} - moguće otkrivanje nastanka kvarnog stanja u samo
pojedinim slučajevima i
\item \textit{Very remote to absolute uncertainty (5) -} gotovo je nemoguće otkriti
nastanak kvarnog stanja.
\end{itemize}
\medskip{}

 \color{green}

The RPN represents the product of these factors (RPN = O$\cdot$S$\cdot$D) and as these factors are in range of 1 to 5, the maximum possible value for RPN is 125. However,  the RPN above 30 is considered as a high priority risk which needs to be further analysed \cite{FTC_ETH_Thomas_Schneider}. Then, these risks can be divided and treated in groups that represent failures which are usually called a risk reduction group.
Then, following discussion will be concentrated on these risks reduction groups and failure modes inside these groups that have a highest RPN value. If the resulting analysis of these groups shows that one of the groups has a lot of failure modes with high RPN value we can create redundant components to increase functionality and safety of entire system. In this way the analysis of failure modes is simplified and it is ensured that the minimal required actions are conducted and system is efficiently restored. 

\color{black}

\section{Failure Mode and Effects Analysis for UAV based on electrical motors}

 \color{green}

Detailed description of FMEA for UAV with electric motor is described in \cite{FTC_ETH_Thomas_Schneider}. The steps of conducted analysis are shown in the Fig. \ref{fig:FMEA_koraci}


 Carrying out the above steps author abstracted system's  physical and logical low-level components into functional blocks. The obtained functional block diagram (FBD) is shown in Fig. \ref{fig:UAV_shema}. A detailed focus during this analysis was put both on all logical parts and physical parts of the system. By using the FMEA, the following risk reduction groups have been defined: 1. Propulsion system, 2. Motor communication bus, 3. Flight electronics and 4. Battery. The author has discovered 80 possible failure modes of the system on and their subsystem of UAV with electrical motor, 43 of them have RPN above of 30 and represent components with high priority risks. A high RPN number have the failure modes related to the fault of components  including: power supply, accelerometers, gyroscopes, brushless engine controller, magnetometers and flight control electronics. 

\color{black}


\begin{figure}[H]
\centering{}\includegraphics[scale=0.7]{chapters/Chapter6/FMEA_analiza.pdf}
\caption{{Koraci u provodjenje FME analize \cite{FTC_ETH_Thomas_Schneider}.
\label{fig:FMEA_koraci}}}
\end{figure}


Provodeći korake FME analize prikazane na slici \ref{fig:FMEA_koraci}
autor je cijeli sustav bespilotne letjelice podijelio u funkcionalne
blokove ({\emph{engl.}} Functional Block
Diagram - FBD) koji predstavljaju fizičke i logičke cjeline sustava.
Prikaz fizičkih i logičkih cjelina sustava predočen je na slici \ref{fig:UAV_shema}.


\begin{figure}[H]
\centering{}\includegraphics[scale=0.45]{chapters/Chapter6/Slika_04.pdf}
\caption{{Structure of multirotor \cite{FTC_ETH_Thomas_Schneider}.
\label{fig:UAV_shema}}}
\end{figure}








Kao što se može vidjeti na slici \ref{fig:UAV_shema}, sustav bespilotne
letjelice podijeljen je u neovisne funkcionalne blokove: fizički dio
sustava (aktuatori, senzori, baterija), logički dio sustava (algoritmi
za estimaciju stanja, planiranje misije te upravljački algoritam)
i mehanički dio sustava (pod nazivom višerotorski sustav). Mehanički
dio sustava prikazan je jednim blokom, jer za slučaj da dodje do strukturalnog
kvara nema načina da se učinkovito djeluje bilo kakvom akcijom. Izmedju
funkcionalnih blokova dana je medjusobna ovisnost u vidu linija koje
ih povezuju. 


Sljedeći je korak definiranje nazivnog radnog režima za bespilotnu
letjelicu. Za potrebe analize pretpostavlja se da nazivni radni režim
podrazumijeva sljedeće:

\color{red}

\medskip{}
\begin{itemize}
\item Multirotor is flying in autopilot mode or in manual 
ight,
\item Safety pilot is available and in range, in case of an emergency switch to manual mode,
\item No obstacles in the near surroundings of the MAV,
\item No or only calm / steady wind.
\end{itemize}

\color{black}



\color{green}

The author has discovered 80 possible failure modes of the system on and their subsystem of UAV with electrical motor, 43 of them have RPN above of 30 and represent components with high priority risks ($RPN>30$). In table \ref{tab:FMEA_UAV} are show a part of the fault states with a high RPN number



\color{black}

\medskip{}








\begin{table*}[!t]
\caption{Part of High Priority Risks table from \cite{FTC_ETH_Thomas_Schneider} }
\label{tab:FMEA_UAV}
\begin{center}
{\small
 \begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{FMEA resulting table for fuel tank}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
  & \multicolumn{1}{c|}{Failure mode}                                                         & \multicolumn{1}{c|}{Effect}                                                                                                                                                                               & Cause(s)                                                                                & \multicolumn{1}{c|}{Possible action}                                                                     & \multicolumn{1}{l|}{RPN} \\ \hline
\begin{tabular}[c]{@{}l@{}}A.301 \\ battery \end{tabular} & \begin{tabular}[c]{@{}l@{}}discharging \\ under the  \\operating\\ voltage \end{tabular} & \begin{tabular}[c]{@{}l@{}}loss of power  \\ (inactivation of \\the system) \end{tabular}                                                        & \begin{tabular}[c]{@{}c@{}}bad battery \\ level monitoring,\\ user ignores alert\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}measuring\\ voltage/ \\ and  \\alert user\end{tabular}} & 50                       \\ \hline
\begin{tabular}[c]{@{}l@{}}A.302 \\ battery \end{tabular} & failure of battery                                                                         & \begin{tabular}[c]{@{}l@{}}loss of power  \\ (inactivation of \\the system) \end{tabular}                                                 & \multicolumn{1}{c|}{damaged battery}                                            & \begin{tabular}[c]{@{}c@{}}  none \end{tabular} & 50                       
 \\ \hline
\begin{tabular}[c]{@{}l@{}}C.101 \\ flight  \\ elect. \end{tabular} &  \begin{tabular} low/\\ high/\\ no output \end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}low battery\\ voltage \end{tabular} & \begin{tabular}no power supply \\ for components\end{tabular} & \begin{tabular}[c]{@{}c@{}} none \end{tabular}                                                                         & 50                      
 \\ \hline
\begin{tabular}[c]{@{}l@{}}G.201 \\ DC \\ motor \end{tabular} & MCU crash                                                                    & \begin{tabular}[c]{@{}l@{}}software\\ error \end{tabular} &\begin{tabular}[c]{@{}l@{}} failure of \\the propulsion \\unit \\ short circuit\\of the battery \end{tabular} & \begin{tabular}[c]{@{}c@{}} none \end{tabular}                                                                         & 50          
  \\ \hline
\begin{tabular}[c]{@{}l@{}}E.201 \\ gyros \end{tabular} & no signal & \begin{tabular}[c]{@{}l@{}}sampling failure \end{tabular} &\begin{tabular}[c]{@{}l@{}} fast attitude\\ changes \\ control can be\\ unstable \end{tabular} & \begin{tabular}[c]{@{}c@{}} none \end{tabular}                                                                         & 50  
  \\ \hline
\begin{tabular}[c]{@{}l@{}}A.402 \\ prop. \end{tabular} &  \begin{tabular}[c]{@{}c@{}}deviation from \\desired torque \end{tabular} & \begin{tabular}[c]{@{}l@{}}loss of control \end{tabular} &\begin{tabular}[c]{@{}l@{}} partial rotor\\ damage \\ loss of motor\end{tabular} & \begin{tabular}[c]{@{}c@{}} adaptive \\ control \end{tabular}                                                                         & 48    \\ \hline
\end{tabular}
  }
\end{center}
\end{table*}

\color{green}

By using the FMEA, the following risk reduction groups have been defined (table \ref{tab:FMEA_UAV}) :





\medskip{}
\begin{itemize}
\item Propulsion system,
\item Motor communication bus, 
\item Flight electronics and
\item Battery.
\end{itemize}
\medskip{}



 \color{green}

Part of the table that cointains failure modes with high RPN values presented by the author in \cite{FTC_ETH_Thomas_Schneider} is shown in Table \ref{tab:FMEA_UAV}. In the table the author shows part of the system to which is the failure mode related, \textit{Failure mode}-type of failure mode, \textit{Effect}-effects of the failure mode to entire system, \textit{Cause(s)}-possible part of system that causes failure mode, \textit{Possible action}-actions to overcome the failure mode. As it can be seen from  Table \ref{tab:FMEA_UAV}, the failure mode which is directly related to a possible control issue was related to the battery voltage, propulsion  and sensors systems.

It is possible to perform certain improvements  of these components to decrease the RPN value under 30, and to improve functionality and security of the overall system. The author has used a fault control technique to improve the RPN values for the failure modes related to the propulsion system and stabilization control categories.  




A high RPN number have the failure modes related to the fault of components  including:    




\medskip{}
\begin{itemize}
\item power supply,
\item accelerometers,
\item gyroscopes,
\item  magnetometers
\item brushless engine controller and
\item flight control electronics. 
\end{itemize}
\medskip{}

\color{black}

Od pobrojanih komponenata veći se dio odnosi na senzore i upravljačku
elektroniku. Kako se radi o komponentama koje dopuštaju redundanciju
to se uvodjenjem dodatnih senzora i upravljačke elektronike može povećati
pouzdanost sustava kako je to napravljeno u radu \cite{osmic_FMEA}. 


\begin{figure}[H]
\centering{}\includegraphics[scale=0.45]{chapters/Chapter6/UAV_redudanca.pdf}
\caption{Structure of system for control and communication
\cite{osmic_FMEA}.\label{fig:UAV_redundancija}}
\end{figure}

\color{blue}

 Namely, the control algorithm is implemented throughout two stages, the one for lower control level (implemented on Pixhawk), and the one for planning level (implemented on Intel Nuc platform). In the proposed design, there were two Pixhawk units which are connected in parallel, where each unit has its own sensors (3x accelerometer, 3x gyroscope, 3x magnetometer, 2x barometer). The implemented redundancy certainly addressed the problems the previous FMEA has shown, and ensured the failure modes related to the used sensors and flight control electronics have now much smaller RPN values for sensors and control electronics for UAV.
After the detailed FMEA, the author conducted experimental system testing. During these tests the author discovered that the two main problems are related to: \textit{battery voltage} (battery voltage rapidly changes while discharging and cause problems with motor control and sensor system) and \textit{control of DC motors} (unstable rotor speed or motors jamming in place). 
\color{black}





Ako nosivost
sustava bespilotne letjelice to može dopustiti, onda se može koristiti
dodatna baterija.
\color{blue}

The risk of a failure in the propulsion system should be considered with the highest priority level. 
\color{black}
Ostaje još razmotriti problem vezan za propulziju
kod bespilotnih letjelica. Kao jedan od mogućih načina snižavanja
$RPN$ broja vezana za propulziju autor predlaže: (i) korištenje bespilotne
letjelice koja ima više pogonskih motora nego što je neophodno za
generiranje referentnog upravljačkog signala (heksakopter ili oktokopter),
(ii) pažljiv odabir smjerova vrtnje pogonskih motora, (iii) korištenje
tehnike za identifikaciju nastanka kvarnog stanja i (iv) upravljanje
koje se može svojom strukturom prilagoditi na nastanak kvarnog stanja.

\section{Definiranje mjere za procjenu završetka misije}


FME analiza koja je provedena u prethodnom potpoglavlju može ukazati
koji od pojedinih dijelova sustava mogu biti kritični za sustav u
cjelini. Nakon što se provede potrebna analiza i odrede kritične komponente
u sustavu može se pristupiti odredjenim akcijama za smanjenje $RPN$
broja za pojedine kritične komponente, te tako dobiti pouzdaniji sustav.
U prethodnim je poglavljima disertacije takodjer pokazano da mogućnost
letjelice da prati referentnu trajektoriju, a samim time izvršava
planiranu misiju, ovisi o upravljanju koje joj je na raspolaganju,
bez obzira na posjedovanje redundantne strukture. Takodjer u analizi
koja je provedena za utjecaj broja motora kao i smjera njihove vrtnje,
pokazano je da su odredjene strukture otpornije od drugih za slučaj
jednostrukog i dvostrukog kvarnog stanja na motorima. Ako bi se i
planiranje misije izvelo tako da se uvaže mogućnosti nastanka kvarnog
stanja tada bi imali i planiranje koje je prilagodjeno odabranoj strukturi
i kvarnim stanjima koji mogu nastati na strukturi bespilotne letjelice.
Uvažavajući sve navedene činjenice, možemo definirati $RPN$ broj
za procjenu završetka misije koji se računa kao $RPN=L\cdot U\ensuremath{\cdot}K\ensuremath{\cdot}P$,
gdje su 


\medskip{}
\begin{itemize}
\item $L$- tip korištene letjelice,
\item $U$- upravljanje primijenjeno na bespilotnoj letjelici,
\item $K$- tip kvarnog stanja i
\item $P$- planiranje misije prilagodjeno nastanku kvarnog stanja.
\end{itemize}
\medskip{}
\textbf{\textit{Tip korištene letjelice (L)}} podijeljen je u pet
kategorija: 

\medskip{}
\begin{itemize}
\item \textit{višerotorski sustav s brojem rotora $\ensuremath{\geqslant}10$
}- brojčana vrijednost (1),
\item \textit{oktokopter PPNNPPNN }- brojčana vrijednost (2),
\item \textit{oktokopter PNPNPNPN} - brojčana vrijednost (3), 
\item \textit{heksakopter} - brojčana vrijednost (4) i
\item \textit{kvadkopter} - brojčana vrijednost (5).
\end{itemize}
\medskip{}
\textbf{\textit{Upravljanje primijenjeno na bespilotnoj letjelici
(U)}} podijeljeno je u četiri kategorije:

\medskip{}
\begin{itemize}
\item \textit{prilagodjeno upravljanje -} brojčana vrijednost (1),
\item \textit{djelomično prilagodjeno - }brojčana vrijednost (2),
\item \textit{robusno upravljanje} - brojčana vrijednost (3) i
\item \textit{neprilagodjeno upravljanje} - brojčana vrijednost (4).
\end{itemize}
\medskip{}
\textbf{\textit{Tip kvarnog stanja (K)}} podijeljen je na tri brojčane
vrijednosti (koristimo tablice dobivene analizom utjecaja tipa letjelice
i smjerova vrtnje motora): 

\medskip{}
\begin{itemize}
\item \textit{bez kvarnog stanja -} brojčana vrijednost (1),
\item \textit{jednostruki prilagodljiv - }brojčana vrijednost (1),\textit{ }
\item \textit{jednostruki neprilagodljiv - }brojčana vrijednost (10),
\item \textit{dvostruki prilagodljiv - }brojčana vrijednost \textit{(3)
i} 
\item \textit{dvostruki neprilagodljiv - }brojčana vrijednost\textit{ (10).}
\end{itemize}
\medskip{}
\textbf{\textit{Planiranje misije prilagodjeno nastanku kvarnog stanja
(P) }}podijeljeno je u tri kategorije: 

\medskip{}
\begin{itemize}
\item \textit{potpuno prilagodjeno -} brojčana vrijednost (1),
\item \textit{djelomično prilagodjeno - }brojčana vrijednost (2)\textit{
i}
\item \textit{neprilagodjeno - }brojčana vrijednost (3).
\end{itemize}
\medskip{}

Definiranom mjerom može se procijeniti završetak misije ovisno o tipu
letjelice, korištenom upravljanju, tipu kvarnog stanja i korištenom
planeru gibanja. U najnepovoljnijem slučaju mjera bi dala vrijednost
iznosa 600, medjutim s aspekta sigurnosti i željenog završetka misije
sve vrijednosti iznad 40 bi trebale biti razmotrene. Analogno postupku
FME analize u prethodnom potpoglavlju, potrebno je razmotriti šta
se može učiniti da bi se $RPN$ broj spustio na nižu vrijednost. U
konkretnom slučaju bi se moglo razmisliti o odabiru drugačijeg tipa
letjelice, drugog algoritma upravljanja ili korištenjem pouzdanijih
komponenata na sustavu bespilotne letjelice. Od definiranih faktora
koji tvore mjeru za procjenu završetka misije neophodno je još definirati
planiranje gibanja koje bi u obzir uzelo tip letjelice i tip kvarnog
stanja, što je obradjeno o sljedećem poglavlju.\medskip{}


==> frontmatter/contributor.tex <==
%%\twocolumn
\chapter*{Contributors}

\begin{multicols}{2}
\contributor{Michael Aftosmis}{NASA Ames Research Center}{Moffett Field, California}

\contributor{Pratul K. Agarwal}{Oak Ridge National Laboratory}{Oak Ridge, Tennessee}

\contributor{Sadaf R. Alam}{Oak Ridge National Laboratory}{Oak Ridge, Tennessee}

\contributor{Gabrielle Allen}{Louisiana State University}{Baton Rouge, Louisiana}

\contributor{Martin Sandve Aln{\ae}s}{Simula Research Laboratory and University of Oslo, Norway}{Norway}

\contributor{Steven F. Ashby} {Lawrence Livermore National Laboratory}{Livermore, California}

\contributor{David A. Bader} {Georgia Institute of Technology}{Atlanta, Georgia}

\contributor{Benjamin Bergen} {Los Alamos National Laboratory}{Los Alamos, New Mexico}

\contributor{Jonathan W. Berry} {Sandia National Laboratories}{Albuquerque, New Mexico}

\contributor{Martin Berzins}{University of Utah}{Salt Lake City, Utah}

\contributor{Abhinav Bhatele}{University of Illinois}{Urbana-Champaign, Illinois}

\contributor{Christian Bischof} {RWTH Aachen University}{Germany}

\contributor{Rupak Biswas} {NASA Ames Research Center}{Moffett Field, California}\vspace*{5pt}

\contributor{Eric Bohm} {University of Illinois}{Urbana-Champaign, Illinois}\vspace*{5pt}

\contributor{James Bordner} {University of California, San Diego}{San Diego, California}\vspace*{5pt}

\contributor{George Bosilca} {University of Tennessee}{Knoxville, Tennessee}\vspace*{5pt}

\contributor{Greg L. Bryan} {Columbia University}{New York, New York}\vspace*{5pt}

\contributor{Marian Bubak} {AGH University of Science and Technology}{
Krak{\'o}w, Poland}\vspace*{5pt}

\contributor{Andrew Canning}{Lawrence Berkeley National
Laboratory}{Berkeley, California}

\contributor{Jonathan Carter} {Lawrence Berkeley National
Laboratory}{Berkeley, California}

\contributor{Zizhong Chen} {Jacksonville State University}{Jacksonville,
Alabama}

\contributor{Joseph R. Crobak} {Rutgers, The State University of New
Jersey}{Piscataway, New Jersey}

\contributor{Roxana E. Diaconescu} {Yahoo! Inc.}{Burbank, California}

\contributor{Peter Diener}
{Louisiana State University}{Baton Rouge, Louisiana}

\contributor{Jack J. Dongarra} {University of Tennessee, Knoxville, 
Oak Ridge National Laboratory, and}{University of Manchester}

\contributor{John B. Drake} {Oak Ridge National Laboratory}{Oak Ridge,
Tennessee}

\contributor{Kelvin K. Droegemeier} {University of Oklahoma}{Norman,
Oklahoma}

\contributor{St{\'e}phane Ethier} {Princeton University}{Princeton, New
Jersey}

\contributor{Christoph Freundl}
{Friedrich--Alexander--Universit{\"a}t}{Erlangen, Germany}

\contributor{Karl F{\"u}rlinger} {University of Tennessee}{Knoxville,
Tennessee}

\contributor{Al Geist} {Oak Ridge National Laboratory}{Oak Ridge,
Tennessee}

\contributor{Michael Gerndt} {Technische Universit{\"a}t
M{\"u}nchen}{Munich, Germany}

\contributor{Tom Goodale}
{Louisiana State University}{Baton Rouge, Louisiana}

\contributor{Tobias Gradl}
{Friedrich--Alexander--Universit{\"a}t}{Erlangen, Germany}

\contributor{William D. Gropp} {Argonne National Laboratory}{Argonne,
Illinois}

\contributor{Robert Harkness} {University of California, San
Diego}{San Diego, California}

\contributor{Albert Hartono} {Ohio State University}{Columbus, Ohio}

\contributor{Thomas C. Henderson} {University of Utah}{Salt Lake City,
Utah}

\contributor{Bruce A. Hendrickson} {Sandia National
Laboratories}{Albuquerque, New Mexico}

\contributor{Alfons G. Hoekstra} {University of Amsterdam}{Amsterdam,
The Netherlands}

\contributor{Philip W. Jones} {Los Alamos National Laboratory}{Los
Alamos, New Mexico}

\contributor{Laxmikant Kal{\'e}} {University of
Illinois}{Urbana-Champaign, Illinois}

\contributor{Shoaib Kamil} {Lawrence Berkeley National
Laboratory}{Berkeley, California}

\contributor{Cetin Kiris} {NASA Ames Research Center}{Moffett Field,
California}

\contributor{Uwe K{\"u}ster} {University of Stuttgart}{Stuttgart,
Germany}

\contributor{Julien Langou} {University of Colorado}{Denver, Colorado}

\contributor{Hans Petter Langtangen}
{Simula Research Laboratory and}{University of Oslo, Norway}

\contributor{Michael Lijewski} {Lawrence Berkeley National
Laboratory}{Berkeley, California}

\contributor{Anders Logg}
{Simula Research Laboratory and}{University of Oslo, Norway}

\contributor{Justin Luitjens} {University of Utah}{Salt Lake City, Utah}

\contributor{Kamesh Madduri} {Georgia Institute of Technology}{Atlanta,
Georgia}

\contributor{Kent-Andre Mardal}
{Simula Research Laboratory and}{University of Oslo, Norway}

\contributor{Satoshi Matsuoka} {Tokyo Institute of Technology}{Tokyo,
Japan}

\contributor{John M. May} {Lawrence Livermore National
Laboratory}{Livermore, California}

\contributor{Celso L. Mendes} {University of Illinois}{Urbana-Champaign,
Illinois}

\contributor{Dieter an Mey} {RWTH Aachen University}{Germany}

\contributor{Tetsu Narumi} {Keio University}{Japan}

\contributor{Michael L. Norman} {University of California, San
Diego}{San Diego, California}

\contributor{Boyana Norris} {Argonne National Laboratory}{Argonne,
Illinois}

\contributor{Yousuke Ohno} {Institute of Physical and Chemical Research
(RIKEN)}{Kanagawa, Japan}

\contributor{Leonid Oliker} {Lawrence Berkeley National
Laboratory}{Berkeley, California}

\contributor{Brian O'Shea} {Los Alamos National Laboratory}{Los Alamos,
New Mexico}

\contributor{Christian D. Ott}
{University of Arizona}{Tucson, Arizona}

\contributor{James C. Phillips} {University of
Illinois}{Urbana-Champaign, Illinois}

\contributor{Simon Portegies Zwart} {University of
Amsterdam,}{Amsterdam, The Netherlands}

\contributor{Thomas Radke}
{Albert-Einstein-Institut}{Golm, Germany}

\contributor{Michael Resch} {University of Stuttgart}{Stuttgart,
Germany}

\contributor{Daniel Reynolds} {University of California, San Diego}{San
Diego, California}

\contributor{Ulrich R{\"u}de}
{Friedrich--Alexander--Universit{\"a}t}{Erlangen, Germany}

\contributor{Samuel Sarholz}
{RWTH Aachen University}{Germany}

\contributor{Erik Schnetter}
{Louisiana State University}{Baton Rouge, Louisiana}

\contributor{Klaus Schulten} {University of Illinois}{Urbana-Champaign,
Illinois}

\contributor{Edward Seidel}
{Louisiana State University}{Baton Rouge, Louisiana}

\contributor{John Shalf} {Lawrence Berkeley National
Laboratory}{Berkeley, California}

\contributor{Bo-Wen Shen} {NASA Goddard Space Flight Center}{Greenbelt,
Maryland}

\contributor{Ola Skavhaug}
{Simula Research Laboratory and}{University of Oslo, Norway}

\contributor{Peter M.A. Sloot} {University of Amsterdam}{Amsterdam, The
Netherlands}

\contributor{Erich Strohmaier} {Lawrence Berkeley National
Laboratory}{Berkeley, California}

\contributor{Makoto Taiji} {Institute of Physical and Chemical Research
(RIKEN)}{Kanagawa, Japan}

\contributor{Christian Terboven}
{RWTH Aachen University,}{Germany}

\contributor{Mariana Vertenstein} {National Center for Atmospheric
Research}{Boulder, Colorado}

\contributor{Rick Wagner} {University of California, San Diego}{San
Diego, California}

\contributor{Daniel Weber} {University of Oklahoma}{Norman, Oklahoma}

\contributor{James B. White, III} {Oak Ridge National Laboratory}{Oak
Ridge, Tennessee}

\contributor{Terry Wilmarth} {University of Illinois}{Urbana-Champaign,
Illinois}

\end{multicols}

==> frontmatter/dedication.tex <==
\cleardoublepage
\thispagestyle{empty}
\vspace*{\stretch{1}}
\begin{center}
\Large\itshape
To my dog\\
and my cat.
\end{center}
\vspace{\stretch{2}}

==> frontmatter/foreword.tex <==
\chapter*{Foreword}
I am delighted to introduce the first book on Multimedia Data Mining.  When I came to know about this book project undertaken by two of the most active young researchers in the field, I was pleased that this book is coming in early stage of a field that will need it more than most fields do.  In most emerging research fields, a book can play a significant role in bringing some maturity to the field.  Research fields advance through research papers.  In research papers, however, only a limited perspective could be provided about the field, its application potential, and the techniques required and already developed in the field.  A book gives such a chance.  I liked the idea that there will be a book that will try to unify the field by bringing in disparate topics already available in several papers that are not easy to find and understand.  I was supportive of this book project even before I had seen any material on it.  The project was a brilliant and a bold idea by two active researchers.  Now that I have it on my screen, it appears to be even a better idea.  

Multimedia started gaining recognition in 1990s as a field.  Processing, storage, communication, and capture and display technologies had advanced enough that researchers and technologists started building approaches to combine information in multiple types of signals such as audio, images, video, and  text.  Multimedia computing and communication techniques recognize correlated information in multiple sources as well as insufficiency of information in any individual source.    By properly selecting sources to provide complementary information, such systems aspire, much like human perception system, to create a holistic picture of a situation using only partial information from separate sources.

Data mining is a direct outgrowth of progress in data storage and processing speeds.  When it became possible to store large volume of data and run different statistical computations to explore all possible and even unlikely correlations among data, the field of data mining was born.  Data mining allowed people to hypothesize relationships among data entities and explore support for those.  This field has been put to applications in many diverse domains and keeps getting more applications.  In fact many new fields are direct outgrowth of data mining and it is likely to become a powerful computational tool.\vadjust{\vfill\pagebreak}




==> frontmatter/preface.tex <==
\chapter*{Preface}
Approximately 17 million people in the USA (6{\%} of the
population) and 140 million people worldwide (this number is
expected to rise to almost 300 million by the year 2025) suffer
from \textit{diabetes mellitus}. Currently, there a few dozens of
commercialised devices for detecting blood glucose levels [1].
However, most of them are invasive. The development of a
noninvasive method would considerably improve the quality of life
for diabetic patients, facilitate their compliance for glucose
monitoring, and reduce complications and mortality associated with
this disease. Noninvasive and continuous monitoring of glucose
concentration in blood and tissues is one of the most challenging
and exciting applications of optics in medicine. The major
difficulty in development and clinical application of optical
noninvasive blood glucose sensors is associated with very low
signal produced by glucose molecules. This results in low
sensitivity and specificity of glucose monitoring by optical
methods and needs a lot of efforts to overcome this difficulty.

A wide range of optical technologies have been designed in
attempts to develop robust noninvasive methods for glucose
sensing. The methods include infrared absorption, near-infrared
scattering, Raman, fluorescent, and thermal gradient
spectroscopies, as well as polarimetric, polarization
heterodyning, photonic crystal, optoacoustic, optothermal, and
optical coherence tomography (OCT) techniques [1-31].

For example, the polarimetric quantification of glucose is based
on the phenomenon of optical rotatory dispersion, whereby a chiral
molecule in an aqueous solution rotates the plane of linearly
polarized light passing through the solution. The angle of
rotation depends linearly on the concentration of the chiral
species, the pathlength through the sample, and the molecule
specific rotation. However, polarization sensitive optical
technique makes it difficult to measure \textit{in vivo} glucose
concentration in blood through the skin because of the strong
light scattering which causes light depolarization. For this
reason, the anterior chamber of the eye has been suggested as a
sight well suited for polarimetric measurements, since scattering
in the eye is generally very low compared to that in other
tissues, and a high correlation exists between the glucose in the
blood and in the aqueous humor. The high accuracy of anterior eye
chamber measurements is also due to the low concentration of
optically active aqueous proteins within the aqueous humor.

On the other hand, the concept of noninvasive blood glucose
sensing using the scattering properties of blood and tissues as an
alternative to spectral absorption and polarization methods for
monitoring of physiological glucose concentrations in diabetic
patients has been under intensive discussion for the last decade.
Many of the considered  effects, such as changing of the size,
refractive index, packing, and aggregation of RBC under glucose
variation, are important for glucose monitoring in diabetic
patients. Indeed, at physiological concentrations of glucose,
ranging from 40 to 400 mg/dl, the role of some of the effects may
be modified, and some other effects, such as glucose penetration
inside the RBC and the followed hemoglobin glycation, may be
important [30-32].

Noninvasive determination of glucose was attempted using light
scattering of skin tissue components measured by a
spatially-resolved diffuse reflectance or NIR fre\-quen\-cy-domain
reflectance techniques. Both approaches are based on change in
glucose concentration, which affects the refractive index mismatch
between the interstitial fluid and tissue fibers, and hence
reduces scattering coefficient. A glucose clamp experiment showed
that reduced scattering coefficient measured in the visible range
qualitatively tracked changes in blood glucose concentration for
the volunteer with diabetes studied.





==> frontmatter/symbollist.tex <==
\chapter*{Symbols}
\begin{symbollist}{000000}
\symbolentry{$\alpha$}{To solve the generator maintenance scheduling, in the  past, several mathematical techniques have  been applied.}
\symbolentry{$\sigma^2$}{These include integer programming, integer linear programming, dynamic programming, branch and bound etc.}
\symbolentry{$\sum$}{Several heuristic search algorithms have also been developed. In recent years expert systems,}
\symbolentry{$abc$}{fuzzy approaches, simulated annealing and genetic algorithms have also been tested.}
\symbolentry{$\theta\sqrt{abc}$}{This paper presents a survey of the literature}
\symbolentry{$\zeta$}{ over the past fifteen years in the generator}
\symbolentry{$\partial$}{maintenance scheduling. The objective is to}
\symbolentry{sdf}{present a clear picture of the available recent literature}
\symbolentry{ewq}{of the problem, the constraints and the other aspects of}
\symbolentry{bvcn}{the generator maintenance schedule.}
\end{symbollist}
